Priorities in tock-CSP

The $tock$-CSP encoding embeds a rich and flexible approach to modelling discrete timed behaviours in CSP where the event $tock$ is interpreted to mark the passage of time. The model checker FDR provides tailored support for $tock$-CSP, including a prioritisation operator that has typically been used to ensure maximal progress, where time only advances after internal activity has stabilised. Prioritisation may also be used on its own right as a modelling construct. Its operational semantics, however, is only congruent over the most discriminating semantic model of CSP: the finite-linear model. To enable sound and compositional reasoning in a $tock$-CSP setting, we calculate a denotational definition for prioritisation. For that we establish a Galois connection between a specialisation of the finite-linear model, with $tock$ and $\checkmark$, that signals termination, as special events, and $\checkmark$-$tock$-CSP, a model for $tock$-CSP that captures termination, deadlines, and is adequate for reasoning about timed refinement. Our results are mechanised using Isabelle/HOL.

==> paper-dot2tex-fig1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,scale=0.8,transform shape]
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw [rounded corners] (8.0bp,8.0bp) -- (8.0bp,194.0bp) -- (166.0bp,194.0bp) -- (166.0bp,8.0bp) -- cycle;
\end{scope}
  \node (CTM) at (124.0bp,176.5bp) [draw,ellipse] {$\mathbf{TTM}$};
  \node (FL) at (194.0bp,101.5bp) [draw,ellipse] {$\mathcal{FL}$};
  \node (CTC) at (126.0bp,26.0bp) [draw,ellipse] {$\tick\text{-}tock$};
  \draw [->,dashed] (CTC) ..controls (151.71bp,37.033bp) and (164.44bp,44.331bp)  .. (173.0bp,54.0bp) .. controls (180.12bp,62.042bp) and (185.17bp,72.889bp)  .. (FL);
  \draw (200.5bp,64.0bp) node {$tt2fl$};
  \draw (147.65bp,38.315bp) node {$$};
  \draw (197.61bp,85.794bp) node {$$};
  \draw [->,dashed] (FL) ..controls (166.88bp,90.407bp) and (145.6bp,80.765bp)  .. (140.0bp,74.0bp) .. controls (133.55bp,66.216bp) and (130.07bp,55.583bp)  .. (CTC);
  \draw (156.5bp,64.0bp) node {$fl2tt$};
  \draw (174.99bp,90.293bp) node {$$};
  \draw (120.65bp,42.282bp) node {$$};
  \draw [->] (CTM) ..controls (81.212bp,155.77bp) and (32.31bp,125.83bp)  .. (48.0bp,92.0bp) .. controls (59.174bp,67.909bp) and (83.953bp,49.423bp)  .. (CTC);
  \draw (70.5bp,101.5bp) node {$mkTT1$};
  \draw (101.88bp,163.12bp) node {$$};
  \draw (105.44bp,39.183bp) node {$$};
  \draw [->] (FL) ..controls (166.97bp,112.67bp) and (145.74bp,122.35bp)  .. (140.0bp,129.0bp) .. controls (133.3bp,136.76bp) and (129.37bp,147.45bp)  .. (CTM);
  \draw (161.0bp,139.0bp) node {$fl2ttm$};
  \draw (175.04bp,112.75bp) node {$$};
  \draw (131.1bp,160.69bp) node {$$};
  \draw [->] (CTM) ..controls (157.3bp,167.43bp) and (172.59bp,160.45bp)  .. (182.0bp,149.0bp) .. controls (188.36bp,141.25bp) and (191.41bp,130.57bp)  .. (FL);
  \draw (212.0bp,139.0bp) node {$ttm2fl$};
  \draw (150.79bp,165.49bp) node {$$};
  \draw (187.9bp,117.32bp) node {$$};
  \draw [->] (CTC) ..controls (125.54bp,60.691bp) and (124.7bp,123.96bp)  .. (CTM);
  \draw (146.5bp,101.5bp) node {$unTT1$};
  \draw (131.87bp,42.108bp) node {$$};
  \draw (118.13bp,160.63bp) node {$$};
%
\end{tikzpicture}

